On the generation of Beurling type Carleman ultradifferentiable $C_0$-semigroups by scalar type spectral operators

A characterization of the scalar type spectral generators of Beurling type Carleman ultradifferentiable $C_0$-semigroups is established, the important case of the Gevrey ultradifferentiability is considered in detail, the implementation of the general criterion corresponding to a certain rapidly growing defining sequence is observed.

==> jinfo.tex <==
\jvolume{22}
\jyear{2016}
\jnumber{2}

